A Unified Decision Framework for Phase I Dose-Finding Designs

The purpose of a phase I dose-finding clinical trial is to investigate the toxicity profiles of various doses for a new drug and identify the maximum tolerated dose. Over the past three decades, various dose-finding designs have been proposed and discussed, including conventional model-based designs, new model-based designs using toxicity probability intervals, and rule-based designs. We present a simple decision framework that can generate several popular designs as special cases. We show that these designs share common elements under the framework, such as the same likelihood function, the use of loss functions, and the nature of the optimal decisions as Bayes rules. They differ mostly in the choice of the prior distributions. We present theoretical results on the decision framework and its link to specific and popular designs like mTPI, BOIN, and CRM. These results provide useful insights into the designs and their underlying assumptions, and convey information to help practitioners select an appropriate design.

==> code/table/result_random.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Thu Jun 03 21:58:43 2021
\begin{table}
\centering
%\def\~{\hphantom{0}}
%\begin{minipage}{175mm}
\caption{Simulation results of 1,000 random scenarios. Entries are the
  $\bm{mean}_{\bm{sd}}$ (across the 1,000 scenarios)
  proportion of simulated trials for each 
  design and metric. For example, the first entry $0.60$ means 60\% of
  the trials correctly select the true MTD under the mTPI design. The
  last two metrics Tox. and None Sel. are the percentage of patients
  experienced DLT in all simulated trials and the proportion of
  simulated trials in which no dose is selected as the MTD,
  respectively.}  
\label{table:random_result}
\begin{tabular}{ccccccc}
  \hline
 Metrics & mTPI & mTPI-2 & BOIN/CCD & Int-CRM & CRM & i3+3 \\ 
  \hline
Correct Sel. of MTD & $0.60_{(0.15)}$ & $0.62_{(0.14)}$ & $0.62_{(0.14)}$ & $0.62_{(0.14)}$ & $0.62_{(0.14)}$ & $0.62_{(0.14)}$ \\ 
  Sel. over MTD & $0.10_{(0.11)}$ & $0.11_{(0.11)}$ & $0.12_{(0.12)}$ & $0.12_{(0.12)}$ & $0.11_{(0.11)}$ & $0.11_{(0.11)}$ \\ 
  Pat. at MTD & $0.50_{(0.22)}$ & $0.50_{(0.21)}$ & $0.50_{(0.20)}$ & $0.51_{(0.20)}$ & $0.51_{(0.21)}$ & $0.50_{(0.21)}$ \\ 
  Pat. over MTD & $0.11_{(0.10)}$ & $0.11_{(0.10)}$ & $0.12_{(0.11)}$ & $0.12_{(0.11)}$ & $0.12_{(0.10)}$ & $0.11_{(0.10)}$ \\ 
  Tox. & $0.26_{(0.05)}$ & $0.26_{(0.05)}$ & $0.26_{(0.05)}$ & $0.26_{(0.05)}$ & $0.26_{(0.05)}$ & $0.26_{(0.05)}$ \\ 
  None Sel. & $0.04_{(0.07)}$ & $0.04_{(0.07)}$ & $0.04_{(0.07)}$ & $0.04_{(0.07)}$ & $0.04_{(0.07)}$ & $0.04_{(0.07)}$ \\ 
   \hline
\end{tabular}
%\end{minipage}
%vspace*{6pt}
\end{table}

